Using CSNNs to Perform Event-based Data Processing & Classification on ASL-DVS

Recent advancements in bio-inspired visual sensing and neuromorphic computing have led to the development of various highly efficient bio-inspired solutions with real-world applications. One notable application integrates event-based cameras with spiking neural networks (SNNs) to process event-based sequences that are asynchronous and sparse, making them difficult to handle. In this project, we develop a convolutional spiking neural network (CSNN) architecture that leverages convolutional operations and recurrent properties of a spiking neuron to learn the spatial and temporal relations in the ASL-DVS gesture dataset. The ASL-DVS gesture dataset is a neuromorphic dataset containing hand gestures when displaying 24 letters (A to Y, excluding J and Z due to the nature of their symbols) from the American Sign Language (ASL). We performed classification on a pre-processed subset of the full ASL-DVS dataset to identify letter signs and achieved 100\% training accuracy. Specifically, this was achieved by training in the Google Cloud compute platform while using a learning rate of 0.0005, batch size of 25 (total of 20 batches), 200 iterations, and 10 epochs.

==> sections/base_implement.tex <==


The current model implementation is a convolutional spiking neural network designed for classifying numbers in the N-MNIST dataset. This model was constructed following SNN torch's tutorial for creating a CSNN, serving as a foundational framework that will be adapted for the ASL-DVS dataset ~\cite{b8}. As shown in Figure~\ref{components}, the model architecture consists of a 3-layer neural network with two $5 \times 5$ convolutional layers containing 12 and 32 filters, respectively. Each convolutional layer is followed by a $2 \times 2$ max pooling operation, leading to a LIF output neuron. Layer 3 is a fully connected layer that maps 800 neurons to 10 LIF outputs.

For model training, the Adam optimizer was utilized with a learning rate of 0.02 and beta values of 0.9 and 0.999. However, additional hyperparameter tuning is required. The loss function employed was the Mean Square Error (MSE) of the spike count, calculating the MSE between the correct and incorrect spike count estimates. These estimates are typically expressed as proportions of spikes over the total number of time steps. The target proportions for the loss function can vary, but a common choice is an 80\% correct rate and a 20\% incorrect rate, consistent with the baseline implementation~\cite{b8}.

To perform backpropagation using spikes, a specific method known as BackPropagation Through Time (BPTT) was utilized. This algorithm computes gradients by determining the loss of all descendants in the computational graph and aggregating them. Consequently, the derivative of the loss with respect to the weights $\frac{\partial \mathcal{L}}{\partial W}$ is computed for each time step. The equation below illustrates how backpropagation computes this derivative ~\cite{b8}:


\begin{equation}
    \frac{\partial \mathcal{L}}{\partial W} = \sum_{t}\frac{\partial \mathcal{L}(t)}{\partial W} = \sum_{t}\sum_{t\le s}\frac{\partial \mathcal{L}(t)}{\partial W(s)}\frac{\partial \mathcal{W}(s)}{\partial W}
\end{equation}


This allows for the model to learn the parameters, but there is still the problem of calculating the gradients when spikes themselves are non-differentiable (also, called "dead neuron problem"). One popular solution to this is known as the surrogate gradient method. Essentially, this swaps the non-differentiable function for one that is differentiable during the calculation of gradients.



In Figure~\ref{prediction}, the CSNN model is trained on the N-MNIST dataset for 1 epoch and 200 iterations. To accommodate resource constraints, we trained the model using a Google Colaboratory notebook with an A100 GPU, achieving a training accuracy of 93.75\%. To perform a quick check, a test image of label 3  was passed into the model. As illustrated in the figure, the model correctly identified the image, as the spike counts for label 3 increased the most over time. We intend to use this validation approach when testing our updated model for ASL-DVS gesture classification.


\begin{figure}
     \centering
     \includegraphics[width=1\linewidth]{figures/CSNN.png}
     \caption{Model of CSNN Network Architecture}
     \label{components}
 \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/prediction.png}
    \caption{CSNN prediction after 300 timesteps}
    \label{prediction}
\end{figure}


==> sections/base_select.tex <==
\subsection{Dataset Characteristics}

\subsubsection{N-MNIST}
The N-MNIST dataset is the same as the MNIST dataset with 60,000 training images and 10,000 testing images. There are 10 classes representing the digits 0 to 9, each image is 34x34. To convert the MNIST dataset to a neuromorphic dataset, an ATIS sensor mounted on a motorized pan-tilt platform was used to put the DVS camera in motion while pointing at an LCD monitor showing the MNIST images~\cite{b12}. 

Because the dataset contains small images, it provides an opportunity to experiment with CSNNs to gain a deeper understanding of spike encoding and interpretation for classification purposes. Once we have developed a model that achieves high accuracy in classification, we will adapt the network for the ASL-DVS dataset.


\subsubsection{ASL-DVS}
 
The ASL-DVS dataset was created using the IniVation DAVIS240C NVS event-based camera under constant lighting conditions, which captures at a $240 \times 180$ resolution and has a 12 µs latency~\cite{b22}. The events are captured and stored in the AEDAT 2.0 format, but a conversion process is used to achieve AEDAT 4.0, the newest AEDAT format that allows for the usage of the IniVation DV Processing software framework. Using this software, the AEDAT files were converted to CSV files to better view the event-based information and perform data exploration. 

This dataset contains samples from five subjects who signed each letter of the alphabet, besides J and Z. The ASL for J and Z are excluded from the dataset due to the nature of how those letters are signed (includes hand motion along with gesture). In this project, the first four subjects are used to train the CSNN. Figure~\ref{components} demonstrates the breakdown of the ASL-DVS dataset. There are a total of 100,800 samples, each having a duration of approximately 100 milliseconds. There are a varying number of samples for each letter in each subject and each sample has a varying number of events detected by the DVS camera. 

Each event has four attributes: timestamp, x, y, and polarity. The timestamp denotes the exact $\mu$s that this event took place in the specified pixel via x and y coordinates. Lastly, polarity denotes whether there is an increase or decrease in the pixel brightness or intensity, eventually to be encoded as a spike.


\subsection{Dataset Exploration}
To visualize the N-MNIST dataset, we use the Tonic library to load the N-MNIST dataset. Then, we utilize the \texttt{plot\_event\_grid} function to plot an example image. Figure~\ref{nmnist} shows an example of the digit 3 as a neuromorphic version of the MNIST image.

To visualize the ASL-DVS dataset, we used the DV-Processing software to load each subject and each letter in the AEDAT4.0 format. The library contains classes that load in each sample as a batch of events, which renders an image as shown in Figure~\ref{asl_f}. This particular sample contains 1,515 events, creating the silhouette of Subject 1's hand signing the letter 'f' as they move it in an oscillating left-to-right motion. The DVS camera picks up all black pixels in the image, however, in the AEDAT files, the polarity field denotes them as either 0 or 1. This signifies that at the specific pixel, either there was a decrease or increase in pixel brightness. For the sake of visualization and ease of use for the SNN model, we encode all events that occur as 1 (black pixels) while the rest are encoded as 0 (white space).

\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/nmnist.png}
        \caption{N-MNIST}
        \label{nmnist}
    \end{subfigure}
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/subject1_f_frame1.png}
        \caption{ASL-DVS}
        \label{asl_f}
    \end{subfigure}
    \caption{}
    \label{datasets}
\end{figure}


